Electroweak corrections to W-boson pair production at the LHC

Vector-boson pair production ranks among the most important Standard-Model benchmark processes at the LHC, not only in view of on-going Higgs analyses. These processes may also help to gain a deeper understanding of the electroweak interaction in general, and to test the validity of the Standard Model at highest energies. In this work, the first calculation of the full one-loop electroweak corrections to on-shell W-boson pair production at hadron colliders is presented. We discuss the impact of the corrections on the total cross section as well as on relevant differential distributions. We observe that corrections due to photon-induced channels can be amazingly large at energies accessible at the LHC, while radiation of additional massive vector bosons does not influence the results significantly.

==> diags/diaguuWWVF.tex <==
\unitlength=1.5bp%
\begin{center}
\begin{small}
\begin{feynartspicture}(160,80)(4,2)

\FADiagram{}
\FAProp(0.,15.)(6.,10.)(0.,){/Straight}{1}
\FALabel(2.48771,11.7893)[tr]{$u$}
\FAProp(0.,5.)(6.,10.)(0.,){/Straight}{-1}
\FALabel(3.51229,6.78926)[tl]{$u$}
\FAProp(20.,15.)(14.,10.)(0.,){/Sine}{-1}
\FALabel(16.4877,13.2107)[br]{$W$}
\FAProp(20.,5.)(14.,10.)(0.,){/Sine}{1}
\FALabel(17.5123,8.21074)[bl]{$W$}
\FAProp(10.,10.)(6.,10.)(0.,){/Sine}{0}
\FALabel(8.,8.93)[t]{$V$}
\FAProp(10.,10.)(14.,10.)(0.,){/ScalarDash}{0}
\FALabel(12.,10.82)[b]{$S$}
\FAVert(6.,10.){0}
\FAVert(14.,10.){0}
\FAVert(10.,10.){-1}

\FADiagram{}
\FAProp(0.,15.)(6.,10.)(0.,){/Straight}{1}
\FALabel(2.48771,11.7893)[tr]{$u$}
\FAProp(0.,5.)(6.,10.)(0.,){/Straight}{-1}
\FALabel(3.51229,6.78926)[tl]{$u$}
\FAProp(20.,15.)(14.,10.)(0.,){/Sine}{-1}
\FALabel(16.4877,13.2107)[br]{$W$}
\FAProp(20.,5.)(14.,10.)(0.,){/Sine}{1}
\FALabel(17.5123,8.21074)[bl]{$W$}
\FAProp(10.,10.)(6.,10.)(0.,){/Sine}{0}
\FALabel(8.,8.93)[t]{$V$}
\FAProp(10.,10.)(14.,10.)(0.,){/Sine}{0}
\FALabel(12.,11.07)[b]{$V$}
\FAVert(6.,10.){0}
\FAVert(14.,10.){0}
\FAVert(10.,10.){-1}

\FADiagram{}
\FAProp(0.,15.)(10.,14.)(0.,){/Straight}{1}
\FALabel(5.15423,15.5623)[b]{$u$}
\FAProp(0.,5.)(10.,6.)(0.,){/Straight}{-1}
\FALabel(5.15423,4.43769)[t]{$u$}
\FAProp(20.,15.)(10.,6.)(0.,){/Sine}{-1}
\FALabel(16.8128,13.2058)[br]{$W$}
\FAProp(20.,5.)(10.,14.)(0.,){/Sine}{1}
\FALabel(18.1872,7.70582)[bl]{$W$}
\FAProp(10.,10.)(10.,14.)(0.,){/Straight}{0}
\FALabel(9.18,12.)[r]{$F$}
\FAProp(10.,10.)(10.,6.)(0.,){/Straight}{0}
\FALabel(9.18,8.)[r]{$F$}
\FAVert(10.,14.){0}
\FAVert(10.,6.){0}
\FAVert(10.,10.){-1}

\FADiagram{}
\FAProp(0.,15.)(6.,10.)(0.,){/Straight}{1}
\FALabel(2.48771,11.7893)[tr]{$u$}
\FAProp(0.,5.)(6.,10.)(0.,){/Straight}{-1}
\FALabel(3.51229,6.78926)[tl]{$u$}
\FAProp(20.,15.)(14.,10.)(0.,){/Sine}{-1}
\FALabel(16.4877,13.2107)[br]{$W$}
\FAProp(20.,5.)(14.,10.)(0.,){/Sine}{1}
\FALabel(17.5123,8.21074)[bl]{$W$}
\FAProp(6.,10.)(14.,10.)(0.,){/Sine}{0}
\FALabel(10.,8.93)[t]{$V$}
\FAVert(6.,10.){0}
\FAVert(14.,10.){-1}

\FADiagram{}
\FAProp(0.,15.)(10.,14.)(0.,){/Straight}{1}
\FALabel(4.84577,13.4377)[t]{$u$}
\FAProp(0.,5.)(10.,6.)(0.,){/Straight}{-1}
\FALabel(5.15423,4.43769)[t]{$u$}
\FAProp(20.,15.)(10.,6.)(0.,){/Sine}{-1}
\FALabel(16.8128,13.2058)[br]{$W$}
\FAProp(20.,5.)(10.,14.)(0.,){/Sine}{1}
\FALabel(17.6872,8.20582)[bl]{$W$}
\FAProp(10.,14.)(10.,6.)(0.,){/Straight}{0}
\FALabel(9.28,10.)[r]{$F$}
\FAVert(10.,14.){0}
\FAVert(10.,6.){-1}

\FADiagram{}
\FAProp(0.,15.)(10.,14.)(0.,){/Straight}{1}
\FALabel(4.84577,13.4377)[t]{$u$}
\FAProp(0.,5.)(10.,6.)(0.,){/Straight}{-1}
\FALabel(5.15423,4.43769)[t]{$u$}
\FAProp(20.,15.)(10.,6.)(0.,){/Sine}{-1}
\FALabel(16.8128,13.2058)[br]{$W$}
\FAProp(20.,5.)(10.,14.)(0.,){/Sine}{1}
\FALabel(17.6872,8.20582)[bl]{$W$}
\FAProp(10.,14.)(10.,6.)(0.,){/Straight}{0}
\FALabel(9.28,10.)[r]{$F$}
\FAVert(10.,6.){0}
\FAVert(10.,14.){-1}

\FADiagram{}
\FAProp(0.,15.)(6.,10.)(0.,){/Straight}{1}
\FALabel(2.48771,11.7893)[tr]{$u$}
\FAProp(0.,5.)(6.,10.)(0.,){/Straight}{-1}
\FALabel(3.51229,6.78926)[tl]{$u$}
\FAProp(20.,15.)(14.,10.)(0.,){/Sine}{-1}
\FALabel(16.4877,13.2107)[br]{$W$}
\FAProp(20.,5.)(14.,10.)(0.,){/Sine}{1}
\FALabel(17.5123,8.21074)[bl]{$W$}
\FAProp(6.,10.)(14.,10.)(0.,){/Sine}{0}
\FALabel(10.,8.93)[t]{$V$}
\FAVert(14.,10.){0}
\FAVert(6.,10.){-1}

\FADiagram{}
\FAProp(0.,15.)(10.,10.)(0.,){/Straight}{1}
\FALabel(2.48771,11.7893)[tr]{$u$}
\FAProp(0.,5.)(10.,10.)(0.,){/Straight}{-1}
\FALabel(3.51229,6.78926)[tl]{$u$}
\FAProp(20.,15.)(10.,10.)(0.,){/Sine}{-1}
\FALabel(16.4877,13.2107)[br]{$W$}
\FAProp(20.,5.)(10.,10.)(0.,){/Sine}{1}
\FALabel(17.5123,8.21074)[bl]{$W$}
\FAVert(10.,10.){-1}


\end{feynartspicture}
\end{small}
\end{center}

==> diags/diaguuWWbox.tex <==
\unitlength=2.3bp%

\begin{center}
\begin{small}
\begin{feynartspicture}(120,120)(3,3)
%\FALabel(33.,69.96)[]{\large $u\quad u\quad \to\quad W\quad W$}

\FADiagram{}
\FAProp(0.,15.)(6.,13.5)(0.,){/Straight}{1}
\FALabel(3.37593,15.2737)[b]{$u$}
\FAProp(0.,5.)(6.,6.5)(0.,){/Straight}{-1}
\FALabel(3.37593,4.72628)[t]{$u$}
\FAProp(20.,15.)(12.,10.)(0.,){/Sine}{-1}
\FALabel(15.6585,13.3344)[br]{$W$}
\FAProp(20.,5.)(12.,10.)(0.,){/Sine}{1}
\FALabel(16.3415,8.3344)[bl]{$W$}
\FAProp(6.,13.5)(6.,6.5)(0.,){/Straight}{0}
\FALabel(5.18,10.)[r]{$F$}
\FAProp(6.,13.5)(12.,10.)(0.,){/Sine}{0}
\FALabel(9.301,12.6089)[bl]{$V$}
\FAProp(6.,6.5)(12.,10.)(0.,){/Sine}{0}
\FALabel(9.301,7.39114)[tl]{$V$}
\FAVert(6.,13.5){0}
\FAVert(6.,6.5){0}
\FAVert(12.,10.){0}

\FADiagram{}
\FAProp(0.,15.)(6.5,13.5)(0.,){/Straight}{1}
\FALabel(3.59853,15.2803)[b]{$u$}
\FAProp(0.,5.)(6.5,6.5)(0.,){/Straight}{-1}
\FALabel(3.59853,4.71969)[t]{$u$}
\FAProp(20.,15.)(13.5,13.5)(0.,){/Sine}{-1}
\FALabel(16.4015,15.2803)[b]{$W$}
\FAProp(20.,5.)(13.5,6.5)(0.,){/Sine}{1}
\FALabel(16.4015,4.71969)[t]{$W$}
\FAProp(6.5,13.5)(6.5,6.5)(0.,){/Sine}{0}
\FALabel(5.43,10.)[r]{$V$}
\FAProp(6.5,13.5)(13.5,13.5)(0.,){/Straight}{0}
\FALabel(10.,14.32)[b]{$F$}
\FAProp(6.5,6.5)(13.5,6.5)(0.,){/Straight}{0}
\FALabel(10.,5.68)[t]{$F$}
\FAProp(13.5,13.5)(13.5,6.5)(0.,){/Straight}{0}
\FALabel(14.32,10.)[l]{$F$}
\FAVert(6.5,13.5){0}
\FAVert(6.5,6.5){0}
\FAVert(13.5,13.5){0}
\FAVert(13.5,6.5){0}

\FADiagram{}
\FAProp(0.,15.)(6.5,13.5)(0.,){/Straight}{1}
\FALabel(3.59853,15.2803)[b]{$u$}
\FAProp(0.,5.)(6.5,6.5)(0.,){/Straight}{-1}
\FALabel(3.59853,4.71969)[t]{$u$}
\FAProp(20.,15.)(13.5,13.5)(0.,){/Sine}{-1}
\FALabel(16.4015,15.2803)[b]{$W$}
\FAProp(20.,5.)(13.5,6.5)(0.,){/Sine}{1}
\FALabel(16.4015,4.71969)[t]{$W$}
\FAProp(6.5,13.5)(6.5,6.5)(0.,){/Straight}{0}
\FALabel(5.68,10.)[r]{$F$}
\FAProp(6.5,13.5)(13.5,13.5)(0.,){/Sine}{0}
\FALabel(10.,14.57)[b]{$V$}
\FAProp(6.5,6.5)(13.5,6.5)(0.,){/Sine}{0}
\FALabel(10.,5.43)[t]{$V$}
\FAProp(13.5,13.5)(13.5,6.5)(0.,){/ScalarDash}{0}
\FALabel(14.32,10.)[l]{$S$}
\FAVert(6.5,13.5){0}
\FAVert(6.5,6.5){0}
\FAVert(13.5,13.5){0}
\FAVert(13.5,6.5){0}

\FADiagram{}
\FAProp(0.,15.)(6.5,13.5)(0.,){/Straight}{1}
\FALabel(3.59853,15.2803)[b]{$u$}
\FAProp(0.,5.)(6.5,6.5)(0.,){/Straight}{-1}
\FALabel(3.59853,4.71969)[t]{$u$}
\FAProp(20.,15.)(13.5,13.5)(0.,){/Sine}{-1}
\FALabel(16.4015,15.2803)[b]{$W$}
\FAProp(20.,5.)(13.5,6.5)(0.,){/Sine}{1}
\FALabel(16.4015,4.71969)[t]{$W$}
\FAProp(6.5,13.5)(6.5,6.5)(0.,){/Straight}{0}
\FALabel(5.68,10.)[r]{$F$}
\FAProp(6.5,13.5)(13.5,13.5)(0.,){/Sine}{0}
\FALabel(10.,14.57)[b]{$V$}
\FAProp(6.5,6.5)(13.5,6.5)(0.,){/Sine}{0}
\FALabel(10.,5.43)[t]{$V$}
\FAProp(13.5,13.5)(13.5,6.5)(0.,){/Sine}{0}
\FALabel(14.57,10.)[l]{$V$}
\FAVert(6.5,13.5){0}
\FAVert(6.5,6.5){0}
\FAVert(13.5,13.5){0}
\FAVert(13.5,6.5){0}

\FADiagram{}
\FAProp(0.,15.)(6.5,13.5)(0.,){/Straight}{1}
\FALabel(3.59853,15.2803)[b]{$u$}
\FAProp(0.,5.)(6.5,6.5)(0.,){/Straight}{-1}
\FALabel(3.59853,4.71969)[t]{$u$}
\FAProp(20.,15.)(13.5,6.5)(0.,){/Sine}{-1}
\FALabel(17.9814,13.8219)[br]{$W$}
\FAProp(20.,5.)(13.5,13.5)(0.,){/Sine}{1}
\FALabel(17.8314,6.42814)[tr]{$W$}
\FAProp(6.5,13.5)(6.5,6.5)(0.,){/Sine}{0}
\FALabel(5.43,10.)[r]{$V$}
\FAProp(6.5,13.5)(13.5,13.5)(0.,){/Straight}{0}
\FALabel(10.,14.32)[b]{$F$}
\FAProp(6.5,6.5)(13.5,6.5)(0.,){/Straight}{0}
\FALabel(10.,5.68)[t]{$F$}
\FAProp(13.5,6.5)(13.5,13.5)(0.,){/Straight}{0}
\FALabel(12.68,10.)[r]{$F$}
\FAVert(6.5,13.5){0}
\FAVert(6.5,6.5){0}
\FAVert(13.5,6.5){0}
\FAVert(13.5,13.5){0}

\FADiagram{}
\FAProp(0.,15.)(6.5,13.5)(0.,){/Straight}{1}
\FALabel(3.59853,15.2803)[b]{$u$}
\FAProp(0.,5.)(6.5,6.5)(0.,){/Straight}{-1}
\FALabel(3.59853,4.71969)[t]{$u$}
\FAProp(20.,15.)(13.5,6.5)(0.,){/Sine}{-1}
\FALabel(17.9814,13.8219)[br]{$W$}
\FAProp(20.,5.)(13.5,13.5)(0.,){/Sine}{1}
\FALabel(17.8314,6.42814)[tr]{$W$}
\FAProp(6.5,13.5)(6.5,6.5)(0.,){/Straight}{0}
\FALabel(5.68,10.)[r]{$F$}
\FAProp(6.5,13.5)(13.5,13.5)(0.,){/Sine}{0}
\FALabel(10.,14.57)[b]{$V$}
\FAProp(6.5,6.5)(13.5,6.5)(0.,){/Sine}{0}
\FALabel(10.,5.43)[t]{$V$}
\FAProp(13.5,6.5)(13.5,13.5)(0.,){/ScalarDash}{0}
\FALabel(12.68,10.)[r]{$S$}
\FAVert(6.5,13.5){0}
\FAVert(6.5,6.5){0}
\FAVert(13.5,6.5){0}
\FAVert(13.5,13.5){0}

\FADiagram{}
\FAProp(0.,15.)(6.5,13.5)(0.,){/Straight}{1}
\FALabel(3.59853,15.2803)[b]{$u$}
\FAProp(0.,5.)(6.5,6.5)(0.,){/Straight}{-1}
\FALabel(3.59853,4.71969)[t]{$u$}
\FAProp(20.,15.)(13.5,6.5)(0.,){/Sine}{-1}
\FALabel(17.9814,13.8219)[br]{$W$}
\FAProp(20.,5.)(13.5,13.5)(0.,){/Sine}{1}
\FALabel(17.8314,6.42814)[tr]{$W$}
\FAProp(6.5,13.5)(6.5,6.5)(0.,){/Straight}{0}
\FALabel(5.68,10.)[r]{$F$}
\FAProp(6.5,13.5)(13.5,13.5)(0.,){/Sine}{0}
\FALabel(10.,14.57)[b]{$V$}
\FAProp(6.5,6.5)(13.5,6.5)(0.,){/Sine}{0}
\FALabel(10.,5.43)[t]{$V$}
\FAProp(13.5,6.5)(13.5,13.5)(0.,){/Sine}{0}
\FALabel(12.43,10.)[r]{$V$}
\FAVert(6.5,13.5){0}
\FAVert(6.5,6.5){0}
\FAVert(13.5,6.5){0}
\FAVert(13.5,13.5){0}

\FADiagram{}
\FAProp(0.,15.)(13.5,13.)(0.,){/Straight}{1}
\FALabel(3.41023,15.5279)[b]{$u$}
\FAProp(0.,5.)(6.5,6.)(0.,){/Straight}{-1}
\FALabel(3.48569,4.44802)[t]{$u$}
\FAProp(20.,15.)(6.5,13.)(0.,){/Sine}{-1}
\FALabel(16.5898,15.5279)[b]{$W$}
\FAProp(20.,5.)(13.5,6.)(0.,){/Sine}{1}
\FALabel(16.5143,4.44802)[t]{$W$}
\FAProp(13.5,13.)(6.5,13.)(0.,){/Straight}{0}
\FALabel(10.,12.18)[t]{$F$}
\FAProp(13.5,13.)(13.5,6.)(0.,){/Sine}{0}
\FALabel(14.57,9.5)[l]{$V$}
\FAProp(6.5,6.)(6.5,13.)(0.,){/Straight}{0}
\FALabel(5.68,9.5)[r]{$F$}
\FAProp(6.5,6.)(13.5,6.)(0.,){/Sine}{0}
\FALabel(10.,4.93)[t]{$V$}
\FAVert(13.5,13.){0}
\FAVert(6.5,6.){0}
\FAVert(6.5,13.){0}
\FAVert(13.5,6.){0}

\FADiagram{}
\FAProp(0.,15.)(13.5,13.)(0.,){/Straight}{1}
\FALabel(3.41023,15.5279)[b]{$u$}
\FAProp(0.,5.)(6.5,6.)(0.,){/Straight}{-1}
\FALabel(3.48569,4.44802)[t]{$u$}
\FAProp(20.,15.)(6.5,13.)(0.,){/Sine}{-1}
\FALabel(16.5898,15.5279)[b]{$W$}
\FAProp(20.,5.)(13.5,6.)(0.,){/Sine}{1}
\FALabel(16.5143,4.44802)[t]{$W$}
\FAProp(13.5,13.)(6.5,13.)(0.,){/Sine}{0}
\FALabel(10.,11.93)[t]{$V$}
\FAProp(13.5,13.)(13.5,6.)(0.,){/Straight}{0}
\FALabel(14.32,9.5)[l]{$F$}
\FAProp(6.5,6.)(6.5,13.)(0.,){/Sine}{0}
\FALabel(5.43,9.5)[r]{$V$}
\FAProp(6.5,6.)(13.5,6.)(0.,){/Straight}{0}
\FALabel(10.,5.18)[t]{$F$}
\FAVert(13.5,13.){0}
\FAVert(6.5,6.){0}
\FAVert(6.5,13.){0}
\FAVert(13.5,6.){0}

\end{feynartspicture}
\end{small}
\end{center}


==> diags/diaguuWWse.tex <==
\unitlength=2.3bp%
%\SetScale{2bp}

\begin{center}
\begin{small}
\begin{feynartspicture}(160,80)(4,2)
%\FALabel(33.,69.96)[]{\large $u\quad u\quad \to\quad W\quad W$}

\FADiagram{}
\FAProp(0.,15.)(4.,10.)(0.,){/Straight}{1}
\FALabel(1.26965,12.0117)[tr]{$u$}
\FAProp(0.,5.)(4.,10.)(0.,){/Straight}{-1}
\FALabel(2.73035,7.01172)[tl]{$u$}
\FAProp(20.,15.)(16.,10.)(0.,){/Sine}{-1}
\FALabel(17.2697,12.9883)[br]{$W$}
\FAProp(20.,5.)(16.,10.)(0.,){/Sine}{1}
\FALabel(18.7303,7.98828)[bl]{$W$}
\FAProp(4.,10.)(10.,10.)(0.,){/Sine}{0}
\FALabel(7.,8.93)[t]{$V$}
\FAProp(16.,10.)(10.,10.)(0.,){/Sine}{0}
\FALabel(13.,8.93)[t]{$V$}
\FAProp(10.,10.)(10.,10.)(10.,15.){/ScalarDash}{0}
\FALabel(10.,15.82)[b]{$S$}
\FAVert(4.,10.){0}
\FAVert(16.,10.){0}
\FAVert(10.,10.){0}

\FADiagram{}
\FAProp(0.,15.)(4.,10.)(0.,){/Straight}{1}
\FALabel(1.26965,12.0117)[tr]{$u$}
\FAProp(0.,5.)(4.,10.)(0.,){/Straight}{-1}
\FALabel(2.73035,7.01172)[tl]{$u$}
\FAProp(20.,15.)(16.,10.)(0.,){/Sine}{-1}
\FALabel(17.2697,12.9883)[br]{$W$}
\FAProp(20.,5.)(16.,10.)(0.,){/Sine}{1}
\FALabel(18.7303,7.98828)[bl]{$W$}
\FAProp(4.,10.)(10.,10.)(0.,){/Sine}{0}
\FALabel(7.,8.93)[t]{$V$}
\FAProp(16.,10.)(10.,10.)(0.,){/Sine}{0}
\FALabel(13.,8.93)[t]{$V$}
\FAProp(10.,10.)(10.,10.)(10.,15.){/Sine}{0}
\FALabel(10.,16.07)[b]{$V$}
\FAVert(4.,10.){0}
\FAVert(16.,10.){0}
\FAVert(10.,10.){0}

\FADiagram{}
\FAProp(0.,15.)(3.,10.)(0.,){/Straight}{1}
\FALabel(0.650886,12.1825)[tr]{$u$}
\FAProp(0.,5.)(3.,10.)(0.,){/Straight}{-1}
\FALabel(2.34911,7.18253)[tl]{$u$}
\FAProp(20.,15.)(17.,10.)(0.,){/Sine}{-1}
\FALabel(17.6509,12.8175)[br]{$W$}
\FAProp(20.,5.)(17.,10.)(0.,){/Sine}{1}
\FALabel(19.3491,7.81747)[bl]{$W$}
\FAProp(3.,10.)(7.,10.)(0.,){/Sine}{0}
\FALabel(5.,11.07)[b]{$V$}
\FAProp(17.,10.)(13.,10.)(0.,){/ScalarDash}{0}
\FALabel(15.,9.18)[t]{$S$}
\FAProp(7.,10.)(13.,10.)(0.8,){/Straight}{0}
\FALabel(10.,6.78)[t]{$F$}
\FAProp(7.,10.)(13.,10.)(-0.8,){/Straight}{0}
\FALabel(10.,13.22)[b]{$F$}
\FAVert(3.,10.){0}
\FAVert(17.,10.){0}
\FAVert(7.,10.){0}
\FAVert(13.,10.){0}

\FADiagram{}
\FAProp(0.,15.)(3.,10.)(0.,){/Straight}{1}
\FALabel(0.650886,12.1825)[tr]{$u$}
\FAProp(0.,5.)(3.,10.)(0.,){/Straight}{-1}
\FALabel(2.34911,7.18253)[tl]{$u$}
\FAProp(20.,15.)(17.,10.)(0.,){/Sine}{-1}
\FALabel(17.6509,12.8175)[br]{$W$}
\FAProp(20.,5.)(17.,10.)(0.,){/Sine}{1}
\FALabel(19.3491,7.81747)[bl]{$W$}
\FAProp(3.,10.)(7.,10.)(0.,){/Sine}{0}
\FALabel(5.,11.07)[b]{$V$}
\FAProp(17.,10.)(13.,10.)(0.,){/ScalarDash}{0}
\FALabel(15.,9.18)[t]{$S$}
\FAProp(7.,10.)(13.,10.)(0.8,){/ScalarDash}{0}
\FALabel(10.,6.78)[t]{$S$}
\FAProp(7.,10.)(13.,10.)(-0.8,){/ScalarDash}{0}
\FALabel(10.,13.22)[b]{$S$}
\FAVert(3.,10.){0}
\FAVert(17.,10.){0}
\FAVert(7.,10.){0}
\FAVert(13.,10.){0}

\FADiagram{}
\FAProp(0.,15.)(3.,10.)(0.,){/Straight}{1}
\FALabel(0.650886,12.1825)[tr]{$u$}
\FAProp(0.,5.)(3.,10.)(0.,){/Straight}{-1}
\FALabel(2.34911,7.18253)[tl]{$u$}
\FAProp(20.,15.)(17.,10.)(0.,){/Sine}{-1}
\FALabel(17.6509,12.8175)[br]{$W$}
\FAProp(20.,5.)(17.,10.)(0.,){/Sine}{1}
\FALabel(19.3491,7.81747)[bl]{$W$}
\FAProp(3.,10.)(7.,10.)(0.,){/Sine}{0}
\FALabel(5.,11.07)[b]{$V$}
\FAProp(17.,10.)(13.,10.)(0.,){/ScalarDash}{0}
\FALabel(15.,9.18)[t]{$S$}
\FAProp(7.,10.)(13.,10.)(0.8,){/GhostDash}{0}
\FALabel(10.,6.78)[t]{$U$}
\FAProp(7.,10.)(13.,10.)(-0.8,){/GhostDash}{0}
\FALabel(10.,13.22)[b]{$U$}
\FAVert(3.,10.){0}
\FAVert(17.,10.){0}
\FAVert(7.,10.){0}
\FAVert(13.,10.){0}

\FADiagram{}
\FAProp(0.,15.)(3.,10.)(0.,){/Straight}{1}
\FALabel(0.650886,12.1825)[tr]{$u$}
\FAProp(0.,5.)(3.,10.)(0.,){/Straight}{-1}
\FALabel(2.34911,7.18253)[tl]{$u$}
\FAProp(20.,15.)(17.,10.)(0.,){/Sine}{-1}
\FALabel(17.6509,12.8175)[br]{$W$}
\FAProp(20.,5.)(17.,10.)(0.,){/Sine}{1}
\FALabel(19.3491,7.81747)[bl]{$W$}
\FAProp(3.,10.)(7.,10.)(0.,){/Sine}{0}
\FALabel(5.,11.07)[b]{$V$}
\FAProp(17.,10.)(13.,10.)(0.,){/ScalarDash}{0}
\FALabel(15.,9.18)[t]{$S$}
\FAProp(7.,10.)(13.,10.)(0.8,){/Sine}{0}
\FALabel(10.,6.53)[t]{$V$}
\FAProp(7.,10.)(13.,10.)(-0.8,){/Sine}{0}
\FALabel(10.,13.47)[b]{$V$}
\FAVert(3.,10.){0}
\FAVert(17.,10.){0}
\FAVert(7.,10.){0}
\FAVert(13.,10.){0}

\FADiagram{}
\FAProp(0.,15.)(3.,10.)(0.,){/Straight}{1}
\FALabel(0.650886,12.1825)[tr]{$u$}
\FAProp(0.,5.)(3.,10.)(0.,){/Straight}{-1}
\FALabel(2.34911,7.18253)[tl]{$u$}
\FAProp(20.,15.)(17.,10.)(0.,){/Sine}{-1}
\FALabel(17.6509,12.8175)[br]{$W$}
\FAProp(20.,5.)(17.,10.)(0.,){/Sine}{1}
\FALabel(19.3491,7.81747)[bl]{$W$}
\FAProp(3.,10.)(7.,10.)(0.,){/Sine}{0}
\FALabel(5.,11.07)[b]{$V$}
\FAProp(17.,10.)(13.,10.)(0.,){/ScalarDash}{0}
\FALabel(15.,9.18)[t]{$S$}
\FAProp(7.,10.)(13.,10.)(0.8,){/ScalarDash}{0}
\FALabel(10.,6.78)[t]{$S$}
\FAProp(7.,10.)(13.,10.)(-0.8,){/Sine}{0}
\FALabel(10.,13.47)[b]{$V$}
\FAVert(3.,10.){0}
\FAVert(17.,10.){0}
\FAVert(7.,10.){0}
\FAVert(13.,10.){0}

\FADiagram{}
\FAProp(0.,15.)(3.,10.)(0.,){/Straight}{1}
\FALabel(0.650886,12.1825)[tr]{$u$}
\FAProp(0.,5.)(3.,10.)(0.,){/Straight}{-1}
\FALabel(2.34911,7.18253)[tl]{$u$}
\FAProp(20.,15.)(17.,10.)(0.,){/Sine}{-1}
\FALabel(17.6509,12.8175)[br]{$W$}
\FAProp(20.,5.)(17.,10.)(0.,){/Sine}{1}
\FALabel(19.3491,7.81747)[bl]{$W$}
\FAProp(3.,10.)(7.,10.)(0.,){/Sine}{0}
\FALabel(5.,11.07)[b]{$V$}
\FAProp(17.,10.)(13.,10.)(0.,){/Sine}{0}
\FALabel(15.,8.93)[t]{$V$}
\FAProp(7.,10.)(13.,10.)(0.8,){/Straight}{0}
\FALabel(10.,6.78)[t]{$F$}
\FAProp(7.,10.)(13.,10.)(-0.8,){/Straight}{0}
\FALabel(10.,13.22)[b]{$F$}
\FAVert(3.,10.){0}
\FAVert(17.,10.){0}
\FAVert(7.,10.){0}
\FAVert(13.,10.){0}

\end{feynartspicture}

\unitlength=2.3bp%
\begin{feynartspicture}(120,40)(3,1)
\FADiagram{}
\FAProp(0.,15.)(3.,10.)(0.,){/Straight}{1}
\FALabel(0.650886,12.1825)[tr]{$u$}
\FAProp(0.,5.)(3.,10.)(0.,){/Straight}{-1}
\FALabel(2.34911,7.18253)[tl]{$u$}
\FAProp(20.,15.)(17.,10.)(0.,){/Sine}{-1}
\FALabel(17.6509,12.8175)[br]{$W$}
\FAProp(20.,5.)(17.,10.)(0.,){/Sine}{1}
\FALabel(19.3491,7.81747)[bl]{$W$}
\FAProp(3.,10.)(7.,10.)(0.,){/Sine}{0}
\FALabel(5.,11.07)[b]{$V$}
\FAProp(17.,10.)(13.,10.)(0.,){/Sine}{0}
\FALabel(15.,8.93)[t]{$V$}
\FAProp(7.,10.)(13.,10.)(0.8,){/ScalarDash}{0}
\FALabel(10.,6.78)[t]{$S$}
\FAProp(7.,10.)(13.,10.)(-0.8,){/ScalarDash}{0}
\FALabel(10.,13.22)[b]{$S$}
\FAVert(3.,10.){0}
\FAVert(17.,10.){0}
\FAVert(7.,10.){0}
\FAVert(13.,10.){0}

\FADiagram{}
\FAProp(0.,15.)(3.,10.)(0.,){/Straight}{1}
\FALabel(0.650886,12.1825)[tr]{$u$}
\FAProp(0.,5.)(3.,10.)(0.,){/Straight}{-1}
\FALabel(2.34911,7.18253)[tl]{$u$}
\FAProp(20.,15.)(17.,10.)(0.,){/Sine}{-1}
\FALabel(17.6509,12.8175)[br]{$W$}
\FAProp(20.,5.)(17.,10.)(0.,){/Sine}{1}
\FALabel(19.3491,7.81747)[bl]{$W$}
\FAProp(3.,10.)(7.,10.)(0.,){/Sine}{0}
\FALabel(5.,11.07)[b]{$V$}
\FAProp(17.,10.)(13.,10.)(0.,){/Sine}{0}
\FALabel(15.,8.93)[t]{$V$}
\FAProp(7.,10.)(13.,10.)(0.8,){/GhostDash}{0}
\FALabel(10.,6.78)[t]{$U$}
\FAProp(7.,10.)(13.,10.)(-0.8,){/GhostDash}{0}
\FALabel(10.,13.22)[b]{$U$}
\FAVert(3.,10.){0}
\FAVert(17.,10.){0}
\FAVert(7.,10.){0}
\FAVert(13.,10.){0}

\FADiagram{}
\FAProp(0.,15.)(3.,10.)(0.,){/Straight}{1}
\FALabel(0.650886,12.1825)[tr]{$u$}
\FAProp(0.,5.)(3.,10.)(0.,){/Straight}{-1}
\FALabel(2.34911,7.18253)[tl]{$u$}
\FAProp(20.,15.)(17.,10.)(0.,){/Sine}{-1}
\FALabel(17.6509,12.8175)[br]{$W$}
\FAProp(20.,5.)(17.,10.)(0.,){/Sine}{1}
\FALabel(19.3491,7.81747)[bl]{$W$}
\FAProp(3.,10.)(7.,10.)(0.,){/Sine}{0}
\FALabel(5.,11.07)[b]{$V$}
\FAProp(17.,10.)(13.,10.)(0.,){/Sine}{0}
\FALabel(15.,8.93)[t]{$V$}
\FAProp(7.,10.)(13.,10.)(0.8,){/Sine}{0}
\FALabel(10.,6.53)[t]{$V$}
\FAProp(7.,10.)(13.,10.)(-0.8,){/Sine}{0}
\FALabel(10.,13.47)[b]{$V$}
\FAVert(3.,10.){0}
\FAVert(17.,10.){0}
\FAVert(7.,10.){0}
\FAVert(13.,10.){0}
\end{feynartspicture}

\unitlength=2.3bp%
\begin{feynartspicture}(80,40)(2,1)

\FADiagram{}
\FAProp(0.,15.)(3.,10.)(0.,){/Straight}{1}
\FALabel(0.650886,12.1825)[tr]{$u$}
\FAProp(0.,5.)(3.,10.)(0.,){/Straight}{-1}
\FALabel(2.34911,7.18253)[tl]{$u$}
\FAProp(20.,15.)(17.,10.)(0.,){/Sine}{-1}
\FALabel(17.6509,12.8175)[br]{$W$}
\FAProp(20.,5.)(17.,10.)(0.,){/Sine}{1}
\FALabel(19.3491,7.81747)[bl]{$W$}
\FAProp(3.,10.)(7.,10.)(0.,){/Sine}{0}
\FALabel(5.,11.07)[b]{$V$}
\FAProp(17.,10.)(13.,10.)(0.,){/Sine}{0}
\FALabel(15.,8.93)[t]{$V$}
\FAProp(7.,10.)(13.,10.)(0.8,){/ScalarDash}{0}
\FALabel(10.,6.78)[t]{$S$}
\FAProp(7.,10.)(13.,10.)(-0.8,){/Sine}{0}
\FALabel(10.,13.47)[b]{$V$}
\FAVert(3.,10.){0}
\FAVert(17.,10.){0}
\FAVert(7.,10.){0}
\FAVert(13.,10.){0}

\FADiagram{}
\FAProp(0.,15.)(10.,14.5)(0.,){/Straight}{1}
\FALabel(5.0774,15.8181)[b]{$u$}
\FAProp(0.,5.)(10.,5.5)(0.,){/Straight}{-1}
\FALabel(5.0774,4.18193)[t]{$u$}
\FAProp(20.,15.)(10.,5.5)(0.,){/Sine}{-1}
\FALabel(16.7264,12.9906)[br]{$W$}
\FAProp(20.,5.)(10.,14.5)(0.,){/Sine}{1}
\FALabel(16.7264,7.00942)[tr]{$W$}
\FAProp(10.,14.5)(10.,12.)(0.,){/Straight}{0}
\FALabel(9.18,13.25)[r]{$F$}
\FAProp(10.,5.5)(10.,8.)(0.,){/Straight}{0}
\FALabel(9.18,6.75)[r]{$F$}
\FAProp(10.,12.)(10.,8.)(0.8,){/Straight}{0}
\FALabel(7.58,10.)[r]{$F$}
\FAProp(10.,12.)(10.,8.)(-0.75,){/Sine}{0}
\FALabel(12.0716,10.)[l]{$V$}
\FAVert(10.,14.5){0}
\FAVert(10.,5.5){0}
\FAVert(10.,12.){0}
\FAVert(10.,8.){0}


\end{feynartspicture}
\end{small}
\end{center}



==> diags/diaguuWWtriag.tex <==
\unitlength=2.3bp%

\begin{center}
\begin{small}
\begin{feynartspicture}(160,200)(4,5)
%\FALabel(33.,69.96)[]{\large $u\quad u\quad \to\quad W\quad W$}

\FADiagram{}
\FAProp(0.,15.)(4.,10.)(0.,){/Straight}{1}
\FALabel(1.26965,12.0117)[tr]{$u$}
\FAProp(0.,5.)(4.,10.)(0.,){/Straight}{-1}
\FALabel(2.73035,7.01172)[tl]{$u$}
\FAProp(20.,15.)(16.,13.5)(0.,){/Sine}{-1}
\FALabel(17.4558,15.2213)[b]{$W$}
\FAProp(20.,5.)(16.,6.5)(0.,){/Sine}{1}
\FALabel(17.4558,4.77869)[t]{$W$}
\FAProp(4.,10.)(10.,10.)(0.,){/Sine}{0}
\FALabel(7.,11.07)[b]{$V$}
\FAProp(16.,13.5)(16.,6.5)(0.,){/Straight}{0}
\FALabel(16.82,10.)[l]{$F$}
\FAProp(16.,13.5)(10.,10.)(0.,){/Straight}{0}
\FALabel(12.825,12.3929)[br]{$F$}
\FAProp(16.,6.5)(10.,10.)(0.,){/Straight}{0}
\FALabel(12.825,7.60709)[tr]{$F$}
\FAVert(4.,10.){0}
\FAVert(16.,13.5){0}
\FAVert(16.,6.5){0}
\FAVert(10.,10.){0}

\FADiagram{}
\FAProp(0.,15.)(4.,10.)(0.,){/Straight}{1}
\FALabel(1.26965,12.0117)[tr]{$u$}
\FAProp(0.,5.)(4.,10.)(0.,){/Straight}{-1}
\FALabel(2.73035,7.01172)[tl]{$u$}
\FAProp(20.,15.)(16.,13.5)(0.,){/Sine}{-1}
\FALabel(17.4558,15.2213)[b]{$W$}
\FAProp(20.,5.)(16.,6.5)(0.,){/Sine}{1}
\FALabel(17.4558,4.77869)[t]{$W$}
\FAProp(4.,10.)(10.,10.)(0.,){/Sine}{0}
\FALabel(7.,11.07)[b]{$V$}
\FAProp(16.,13.5)(16.,6.5)(0.,){/ScalarDash}{0}
\FALabel(16.82,10.)[l]{$S$}
\FAProp(16.,13.5)(10.,10.)(0.,){/ScalarDash}{0}
\FALabel(12.825,12.3929)[br]{$S$}
\FAProp(16.,6.5)(10.,10.)(0.,){/ScalarDash}{0}
\FALabel(12.825,7.60709)[tr]{$S$}
\FAVert(4.,10.){0}
\FAVert(16.,13.5){0}
\FAVert(16.,6.5){0}
\FAVert(10.,10.){0}

\FADiagram{}
\FAProp(0.,15.)(4.,10.)(0.,){/Straight}{1}
\FALabel(1.26965,12.0117)[tr]{$u$}
\FAProp(0.,5.)(4.,10.)(0.,){/Straight}{-1}
\FALabel(2.73035,7.01172)[tl]{$u$}
\FAProp(20.,15.)(16.,13.5)(0.,){/Sine}{-1}
\FALabel(17.4558,15.2213)[b]{$W$}
\FAProp(20.,5.)(16.,6.5)(0.,){/Sine}{1}
\FALabel(17.4558,4.77869)[t]{$W$}
\FAProp(4.,10.)(10.,10.)(0.,){/Sine}{0}
\FALabel(7.,11.07)[b]{$V$}
\FAProp(16.,13.5)(16.,6.5)(0.,){/GhostDash}{0}
\FALabel(16.82,10.)[l]{$U$}
\FAProp(16.,13.5)(10.,10.)(0.,){/GhostDash}{0}
\FALabel(12.825,12.3929)[br]{$U$}
\FAProp(16.,6.5)(10.,10.)(0.,){/GhostDash}{0}
\FALabel(12.825,7.60709)[tr]{$U$}
\FAVert(4.,10.){0}
\FAVert(16.,13.5){0}
\FAVert(16.,6.5){0}
\FAVert(10.,10.){0}

\FADiagram{}
\FAProp(0.,15.)(4.,10.)(0.,){/Straight}{1}
\FALabel(1.26965,12.0117)[tr]{$u$}
\FAProp(0.,5.)(4.,10.)(0.,){/Straight}{-1}
\FALabel(2.73035,7.01172)[tl]{$u$}
\FAProp(20.,15.)(16.,13.5)(0.,){/Sine}{-1}
\FALabel(17.4558,15.2213)[b]{$W$}
\FAProp(20.,5.)(16.,6.5)(0.,){/Sine}{1}
\FALabel(17.4558,4.77869)[t]{$W$}
\FAProp(4.,10.)(10.,10.)(0.,){/Sine}{0}
\FALabel(7.,11.07)[b]{$V$}
\FAProp(16.,13.5)(16.,6.5)(0.,){/Sine}{0}
\FALabel(17.07,10.)[l]{$V$}
\FAProp(16.,13.5)(10.,10.)(0.,){/Sine}{0}
\FALabel(12.699,12.6089)[br]{$V$}
\FAProp(16.,6.5)(10.,10.)(0.,){/Sine}{0}
\FALabel(12.699,7.39114)[tr]{$V$}
\FAVert(4.,10.){0}
\FAVert(16.,13.5){0}
\FAVert(16.,6.5){0}
\FAVert(10.,10.){0}

\FADiagram{}
\FAProp(0.,15.)(4.,10.)(0.,){/Straight}{1}
\FALabel(1.26965,12.0117)[tr]{$u$}
\FAProp(0.,5.)(4.,10.)(0.,){/Straight}{-1}
\FALabel(2.73035,7.01172)[tl]{$u$}
\FAProp(20.,15.)(16.,13.5)(0.,){/Sine}{-1}
\FALabel(17.4558,15.2213)[b]{$W$}
\FAProp(20.,5.)(16.,6.5)(0.,){/Sine}{1}
\FALabel(17.4558,4.77869)[t]{$W$}
\FAProp(4.,10.)(10.,10.)(0.,){/Sine}{0}
\FALabel(7.,11.07)[b]{$V$}
\FAProp(16.,13.5)(16.,6.5)(0.,){/ScalarDash}{0}
\FALabel(16.82,10.)[l]{$S$}
\FAProp(16.,13.5)(10.,10.)(0.,){/ScalarDash}{0}
\FALabel(12.825,12.3929)[br]{$S$}
\FAProp(16.,6.5)(10.,10.)(0.,){/Sine}{0}
\FALabel(12.699,7.39114)[tr]{$V$}
\FAVert(4.,10.){0}
\FAVert(16.,13.5){0}
\FAVert(16.,6.5){0}
\FAVert(10.,10.){0}

\FADiagram{}
\FAProp(0.,15.)(4.,10.)(0.,){/Straight}{1}
\FALabel(1.26965,12.0117)[tr]{$u$}
\FAProp(0.,5.)(4.,10.)(0.,){/Straight}{-1}
\FALabel(2.73035,7.01172)[tl]{$u$}
\FAProp(20.,15.)(16.,13.5)(0.,){/Sine}{-1}
\FALabel(17.4558,15.2213)[b]{$W$}
\FAProp(20.,5.)(16.,6.5)(0.,){/Sine}{1}
\FALabel(17.4558,4.77869)[t]{$W$}
\FAProp(4.,10.)(10.,10.)(0.,){/Sine}{0}
\FALabel(7.,11.07)[b]{$V$}
\FAProp(16.,13.5)(16.,6.5)(0.,){/ScalarDash}{0}
\FALabel(16.82,10.)[l]{$S$}
\FAProp(16.,13.5)(10.,10.)(0.,){/Sine}{0}
\FALabel(12.699,12.6089)[br]{$V$}
\FAProp(16.,6.5)(10.,10.)(0.,){/ScalarDash}{0}
\FALabel(12.825,7.60709)[tr]{$S$}
\FAVert(4.,10.){0}
\FAVert(16.,13.5){0}
\FAVert(16.,6.5){0}
\FAVert(10.,10.){0}

\FADiagram{}
\FAProp(0.,15.)(4.,10.)(0.,){/Straight}{1}
\FALabel(1.26965,12.0117)[tr]{$u$}
\FAProp(0.,5.)(4.,10.)(0.,){/Straight}{-1}
\FALabel(2.73035,7.01172)[tl]{$u$}
\FAProp(20.,15.)(16.,13.5)(0.,){/Sine}{-1}
\FALabel(17.4558,15.2213)[b]{$W$}
\FAProp(20.,5.)(16.,6.5)(0.,){/Sine}{1}
\FALabel(17.4558,4.77869)[t]{$W$}
\FAProp(4.,10.)(10.,10.)(0.,){/Sine}{0}
\FALabel(7.,11.07)[b]{$V$}
\FAProp(16.,13.5)(16.,6.5)(0.,){/Sine}{0}
\FALabel(17.07,10.)[l]{$V$}
\FAProp(16.,13.5)(10.,10.)(0.,){/ScalarDash}{0}
\FALabel(12.825,12.3929)[br]{$S$}
\FAProp(16.,6.5)(10.,10.)(0.,){/ScalarDash}{0}
\FALabel(12.825,7.60709)[tr]{$S$}
\FAVert(4.,10.){0}
\FAVert(16.,13.5){0}
\FAVert(16.,6.5){0}
\FAVert(10.,10.){0}

\FADiagram{}
\FAProp(0.,15.)(4.,10.)(0.,){/Straight}{1}
\FALabel(1.26965,12.0117)[tr]{$u$}
\FAProp(0.,5.)(4.,10.)(0.,){/Straight}{-1}
\FALabel(2.73035,7.01172)[tl]{$u$}
\FAProp(20.,15.)(16.,13.5)(0.,){/Sine}{-1}
\FALabel(17.4558,15.2213)[b]{$W$}
\FAProp(20.,5.)(16.,6.5)(0.,){/Sine}{1}
\FALabel(17.4558,4.77869)[t]{$W$}
\FAProp(4.,10.)(10.,10.)(0.,){/Sine}{0}
\FALabel(7.,11.07)[b]{$V$}
\FAProp(16.,13.5)(16.,6.5)(0.,){/ScalarDash}{0}
\FALabel(16.82,10.)[l]{$S$}
\FAProp(16.,13.5)(10.,10.)(0.,){/Sine}{0}
\FALabel(12.699,12.6089)[br]{$V$}
\FAProp(16.,6.5)(10.,10.)(0.,){/Sine}{0}
\FALabel(12.699,7.39114)[tr]{$V$}
\FAVert(4.,10.){0}
\FAVert(16.,13.5){0}
\FAVert(16.,6.5){0}
\FAVert(10.,10.){0}

\FADiagram{}
\FAProp(0.,15.)(4.,10.)(0.,){/Straight}{1}
\FALabel(1.26965,12.0117)[tr]{$u$}
\FAProp(0.,5.)(4.,10.)(0.,){/Straight}{-1}
\FALabel(2.73035,7.01172)[tl]{$u$}
\FAProp(20.,15.)(16.,13.5)(0.,){/Sine}{-1}
\FALabel(17.4558,15.2213)[b]{$W$}
\FAProp(20.,5.)(16.,6.5)(0.,){/Sine}{1}
\FALabel(17.4558,4.77869)[t]{$W$}
\FAProp(4.,10.)(10.,10.)(0.,){/Sine}{0}
\FALabel(7.,11.07)[b]{$V$}
\FAProp(16.,13.5)(16.,6.5)(0.,){/Sine}{0}
\FALabel(17.07,10.)[l]{$V$}
\FAProp(16.,13.5)(10.,10.)(0.,){/ScalarDash}{0}
\FALabel(12.825,12.3929)[br]{$S$}
\FAProp(16.,6.5)(10.,10.)(0.,){/Sine}{0}
\FALabel(12.699,7.39114)[tr]{$V$}
\FAVert(4.,10.){0}
\FAVert(16.,13.5){0}
\FAVert(16.,6.5){0}
\FAVert(10.,10.){0}

\FADiagram{}
\FAProp(0.,15.)(4.,10.)(0.,){/Straight}{1}
\FALabel(1.26965,12.0117)[tr]{$u$}
\FAProp(0.,5.)(4.,10.)(0.,){/Straight}{-1}
\FALabel(2.73035,7.01172)[tl]{$u$}
\FAProp(20.,15.)(16.,13.5)(0.,){/Sine}{-1}
\FALabel(17.4558,15.2213)[b]{$W$}
\FAProp(20.,5.)(16.,6.5)(0.,){/Sine}{1}
\FALabel(17.4558,4.77869)[t]{$W$}
\FAProp(4.,10.)(10.,10.)(0.,){/Sine}{0}
\FALabel(7.,11.07)[b]{$V$}
\FAProp(16.,13.5)(16.,6.5)(0.,){/Sine}{0}
\FALabel(17.07,10.)[l]{$V$}
\FAProp(16.,13.5)(10.,10.)(0.,){/Sine}{0}
\FALabel(12.699,12.6089)[br]{$V$}
\FAProp(16.,6.5)(10.,10.)(0.,){/ScalarDash}{0}
\FALabel(12.825,7.60709)[tr]{$S$}
\FAVert(4.,10.){0}
\FAVert(16.,13.5){0}
\FAVert(16.,6.5){0}
\FAVert(10.,10.){0}

\FADiagram{}
\FAProp(0.,15.)(6.5,14.5)(0.,){/Straight}{1}
\FALabel(3.36888,15.8154)[b]{$u$}
\FAProp(0.,5.)(10.,5.5)(0.,){/Straight}{-1}
\FALabel(5.0774,4.18193)[t]{$u$}
\FAProp(20.,15.)(10.,5.5)(0.,){/Sine}{-1}
\FALabel(13.3251,7.72981)[tl]{$W$}
\FAProp(20.,5.)(13.5,14.5)(0.,){/Sine}{1}
\FALabel(18.4482,8.59123)[bl]{$W$}
\FAProp(10.,5.5)(10.,8.5)(0.,){/Straight}{0}
\FALabel(9.18,7.)[r]{$F$}
\FAProp(6.5,14.5)(13.5,14.5)(0.,){/Straight}{0}
\FALabel(10.,15.32)[b]{$F$}
\FAProp(6.5,14.5)(10.,8.5)(0.,){/Sine}{0}
\FALabel(7.39114,11.199)[tr]{$V$}
\FAProp(13.5,14.5)(10.,8.5)(0.,){/Straight}{0}
\FALabel(12.3181,12.0429)[tl]{$F$}
\FAVert(6.5,14.5){0}
\FAVert(10.,5.5){0}
\FAVert(13.5,14.5){0}
\FAVert(10.,8.5){0}

\FADiagram{}
\FAProp(0.,15.)(6.5,14.5)(0.,){/Straight}{1}
\FALabel(3.36888,15.8154)[b]{$u$}
\FAProp(0.,5.)(10.,5.5)(0.,){/Straight}{-1}
\FALabel(5.0774,4.18193)[t]{$u$}
\FAProp(20.,15.)(10.,5.5)(0.,){/Sine}{-1}
\FALabel(13.3251,7.72981)[tl]{$W$}
\FAProp(20.,5.)(13.5,14.5)(0.,){/Sine}{1}
\FALabel(18.4482,8.59123)[bl]{$W$}
\FAProp(10.,5.5)(10.,8.5)(0.,){/Straight}{0}
\FALabel(9.18,7.)[r]{$F$}
\FAProp(6.5,14.5)(13.5,14.5)(0.,){/Sine}{0}
\FALabel(10.,15.57)[b]{$V$}
\FAProp(6.5,14.5)(10.,8.5)(0.,){/Straight}{0}
\FALabel(7.60709,11.325)[tr]{$F$}
\FAProp(13.5,14.5)(10.,8.5)(0.,){/Sine}{0}
\FALabel(12.5341,11.9169)[tl]{$V$}
\FAVert(6.5,14.5){0}
\FAVert(10.,5.5){0}
\FAVert(13.5,14.5){0}
\FAVert(10.,8.5){0}

\FADiagram{}
\FAProp(0.,15.)(10.,14.5)(0.,){/Straight}{1}
\FALabel(5.0774,15.8181)[b]{$u$}
\FAProp(0.,5.)(6.5,5.5)(0.,){/Straight}{-1}
\FALabel(3.36888,4.18457)[t]{$u$}
\FAProp(20.,15.)(13.5,5.5)(0.,){/Sine}{-1}
\FALabel(18.5763,11.3388)[tl]{$W$}
\FAProp(20.,5.)(10.,14.5)(0.,){/Sine}{1}
\FALabel(13.2922,12.4512)[bl]{$W$}
\FAProp(10.,14.5)(10.,11.5)(0.,){/Straight}{0}
\FALabel(9.28,13.)[r]{$F$}
\FAProp(6.5,5.5)(13.5,5.5)(0.,){/Straight}{0}
\FALabel(10.,4.68)[t]{$F$}
\FAProp(6.5,5.5)(10.,11.5)(0.,){/Sine}{0}
\FALabel(7.39114,8.801)[br]{$V$}
\FAProp(13.5,5.5)(10.,11.5)(0.,){/Straight}{0}
\FALabel(12.7093,7.71415)[bl]{$F$}
\FAVert(10.,14.5){0}
\FAVert(6.5,5.5){0}
\FAVert(13.5,5.5){0}
\FAVert(10.,11.5){0}

\FADiagram{}
\FAProp(0.,15.)(10.,14.5)(0.,){/Straight}{1}
\FALabel(5.0774,15.8181)[b]{$u$}
\FAProp(0.,5.)(6.5,5.5)(0.,){/Straight}{-1}
\FALabel(3.36888,4.18457)[t]{$u$}
\FAProp(20.,15.)(13.5,5.5)(0.,){/Sine}{-1}
\FALabel(18.5763,11.3388)[tl]{$W$}
\FAProp(20.,5.)(10.,14.5)(0.,){/Sine}{1}
\FALabel(13.2922,12.4512)[bl]{$W$}
\FAProp(10.,14.5)(10.,11.5)(0.,){/Straight}{0}
\FALabel(9.28,13.)[r]{$F$}
\FAProp(6.5,5.5)(13.5,5.5)(0.,){/Sine}{0}
\FALabel(10.,4.43)[t]{$V$}
\FAProp(6.5,5.5)(10.,11.5)(0.,){/Straight}{0}
\FALabel(7.60709,8.67503)[br]{$F$}
\FAProp(13.5,5.5)(10.,11.5)(0.,){/Sine}{0}
\FALabel(12.9252,7.84012)[bl]{$V$}
\FAVert(10.,14.5){0}
\FAVert(6.5,5.5){0}
\FAVert(13.5,5.5){0}
\FAVert(10.,11.5){0}

\FADiagram{}
\FAProp(0.,15.)(4.,13.5)(0.,){/Straight}{1}
\FALabel(2.54424,15.2213)[b]{$u$}
\FAProp(0.,5.)(4.,6.5)(0.,){/Straight}{-1}
\FALabel(2.54424,4.77869)[t]{$u$}
\FAProp(20.,15.)(16.,10.)(0.,){/Sine}{-1}
\FALabel(17.2697,12.9883)[br]{$W$}
\FAProp(20.,5.)(16.,10.)(0.,){/Sine}{1}
\FALabel(18.7303,7.98828)[bl]{$W$}
\FAProp(16.,10.)(10.,10.)(0.,){/ScalarDash}{0}
\FALabel(13.,9.18)[t]{$S$}
\FAProp(4.,13.5)(4.,6.5)(0.,){/Straight}{0}
\FALabel(3.18,10.)[r]{$F$}
\FAProp(4.,13.5)(10.,10.)(0.,){/Sine}{0}
\FALabel(7.301,12.6089)[bl]{$V$}
\FAProp(4.,6.5)(10.,10.)(0.,){/Sine}{0}
\FALabel(7.301,7.39114)[tl]{$V$}
\FAVert(4.,13.5){0}
\FAVert(4.,6.5){0}
\FAVert(16.,10.){0}
\FAVert(10.,10.){0}

\FADiagram{}
\FAProp(0.,15.)(4.,13.5)(0.,){/Straight}{1}
\FALabel(2.54424,15.2213)[b]{$u$}
\FAProp(0.,5.)(4.,6.5)(0.,){/Straight}{-1}
\FALabel(2.54424,4.77869)[t]{$u$}
\FAProp(20.,15.)(16.,10.)(0.,){/Sine}{-1}
\FALabel(17.2697,12.9883)[br]{$W$}
\FAProp(20.,5.)(16.,10.)(0.,){/Sine}{1}
\FALabel(18.7303,7.98828)[bl]{$W$}
\FAProp(16.,10.)(10.,10.)(0.,){/Sine}{0}
\FALabel(13.,8.93)[t]{$V$}
\FAProp(4.,13.5)(4.,6.5)(0.,){/Sine}{0}
\FALabel(2.93,10.)[r]{$V$}
\FAProp(4.,13.5)(10.,10.)(0.,){/Straight}{0}
\FALabel(7.17503,12.3929)[bl]{$F$}
\FAProp(4.,6.5)(10.,10.)(0.,){/Straight}{0}
\FALabel(7.17503,7.60709)[tl]{$F$}
\FAVert(4.,13.5){0}
\FAVert(4.,6.5){0}
\FAVert(16.,10.){0}
\FAVert(10.,10.){0}

\FADiagram{}
\FAProp(0.,15.)(4.,13.5)(0.,){/Straight}{1}
\FALabel(2.54424,15.2213)[b]{$u$}
\FAProp(0.,5.)(4.,6.5)(0.,){/Straight}{-1}
\FALabel(2.54424,4.77869)[t]{$u$}
\FAProp(20.,15.)(16.,10.)(0.,){/Sine}{-1}
\FALabel(17.2697,12.9883)[br]{$W$}
\FAProp(20.,5.)(16.,10.)(0.,){/Sine}{1}
\FALabel(18.7303,7.98828)[bl]{$W$}
\FAProp(16.,10.)(10.,10.)(0.,){/Sine}{0}
\FALabel(13.,8.93)[t]{$V$}
\FAProp(4.,13.5)(4.,6.5)(0.,){/Straight}{0}
\FALabel(3.18,10.)[r]{$F$}
\FAProp(4.,13.5)(10.,10.)(0.,){/Sine}{0}
\FALabel(7.301,12.6089)[bl]{$V$}
\FAProp(4.,6.5)(10.,10.)(0.,){/Sine}{0}
\FALabel(7.301,7.39114)[tl]{$V$}
\FAVert(4.,13.5){0}
\FAVert(4.,6.5){0}
\FAVert(16.,10.){0}
\FAVert(10.,10.){0}

\FADiagram{}
\FAProp(0.,15.)(5.,10.)(0.,){/Straight}{1}
\FALabel(1.88398,11.884)[tr]{$u$}
\FAProp(0.,5.)(5.,10.)(0.,){/Straight}{-1}
\FALabel(3.11602,6.88398)[tl]{$u$}
\FAProp(20.,15.)(14.5,13.5)(0.,){/Sine}{-1}
\FALabel(16.8422,15.2654)[b]{$W$}
\FAProp(20.,5.)(12.5,8.)(0.,){/Sine}{1}
\FALabel(15.6743,5.54086)[t]{$W$}
\FAProp(5.,10.)(12.5,8.)(0.,){/Sine}{0}
\FALabel(8.35062,7.98234)[t]{$V$}
\FAProp(14.5,13.5)(12.5,8.)(0.8,){/ScalarDash}{0}
\FALabel(10.5583,11.9943)[r]{$S$}
\FAProp(14.5,13.5)(12.5,8.)(-0.8,){/ScalarDash}{0}
\FALabel(16.4417,9.50573)[l]{$S$}
\FAVert(5.,10.){0}
\FAVert(14.5,13.5){0}
\FAVert(12.5,8.){0}

\FADiagram{}
\FAProp(0.,15.)(5.,10.)(0.,){/Straight}{1}
\FALabel(1.88398,11.884)[tr]{$u$}
\FAProp(0.,5.)(5.,10.)(0.,){/Straight}{-1}
\FALabel(3.11602,6.88398)[tl]{$u$}
\FAProp(20.,15.)(14.5,13.5)(0.,){/Sine}{-1}
\FALabel(16.8422,15.2654)[b]{$W$}
\FAProp(20.,5.)(12.5,8.)(0.,){/Sine}{1}
\FALabel(15.6743,5.54086)[t]{$W$}
\FAProp(5.,10.)(12.5,8.)(0.,){/Sine}{0}
\FALabel(8.35062,7.98234)[t]{$V$}
\FAProp(14.5,13.5)(12.5,8.)(0.8,){/Sine}{0}
\FALabel(10.3233,12.0797)[r]{$V$}
\FAProp(14.5,13.5)(12.5,8.)(-0.8,){/Sine}{0}
\FALabel(16.6767,9.4203)[l]{$V$}
\FAVert(5.,10.){0}
\FAVert(14.5,13.5){0}
\FAVert(12.5,8.){0}

\FADiagram{}
\FAProp(0.,15.)(5.,10.)(0.,){/Straight}{1}
\FALabel(1.88398,11.884)[tr]{$u$}
\FAProp(0.,5.)(5.,10.)(0.,){/Straight}{-1}
\FALabel(3.11602,6.88398)[tl]{$u$}
\FAProp(20.,15.)(12.5,12.)(0.,){/Sine}{-1}
\FALabel(15.6743,14.4591)[b]{$W$}
\FAProp(20.,5.)(14.5,6.5)(0.,){/Sine}{1}
\FALabel(16.8422,4.73462)[t]{$W$}
\FAProp(5.,10.)(12.5,12.)(0.,){/Sine}{0}
\FALabel(8.35062,12.0177)[b]{$V$}
\FAProp(14.5,6.5)(12.5,12.)(0.8,){/ScalarDash}{0}
\FALabel(16.4417,10.4943)[l]{$S$}
\FAProp(14.5,6.5)(12.5,12.)(-0.8,){/ScalarDash}{0}
\FALabel(10.5583,8.00573)[r]{$S$}
\FAVert(5.,10.){0}
\FAVert(14.5,6.5){0}
\FAVert(12.5,12.){0}
\end{feynartspicture}

\begin{feynartspicture}(120,40)(3,1)
\FADiagram{}
\FAProp(0.,15.)(5.,10.)(0.,){/Straight}{1}
\FALabel(1.88398,11.884)[tr]{$u$}
\FAProp(0.,5.)(5.,10.)(0.,){/Straight}{-1}
\FALabel(3.11602,6.88398)[tl]{$u$}
\FAProp(20.,15.)(12.5,12.)(0.,){/Sine}{-1}
\FALabel(15.6743,14.4591)[b]{$W$}
\FAProp(20.,5.)(14.5,6.5)(0.,){/Sine}{1}
\FALabel(16.8422,4.73462)[t]{$W$}
\FAProp(5.,10.)(12.5,12.)(0.,){/Sine}{0}
\FALabel(8.35062,12.0177)[b]{$V$}
\FAProp(14.5,6.5)(12.5,12.)(0.8,){/Sine}{0}
\FALabel(16.6767,10.5797)[l]{$V$}
\FAProp(14.5,6.5)(12.5,12.)(-0.8,){/Sine}{0}
\FALabel(10.3233,7.9203)[r]{$V$}
\FAVert(5.,10.){0}
\FAVert(14.5,6.5){0}
\FAVert(12.5,12.){0}

\FADiagram{}
\FAProp(0.,15.)(4.,10.)(0.,){/Straight}{1}
\FALabel(1.26965,12.0117)[tr]{$u$}
\FAProp(0.,5.)(4.,10.)(0.,){/Straight}{-1}
\FALabel(2.73035,7.01172)[tl]{$u$}
\FAProp(20.,15.)(15.5,10.)(0.,){/Sine}{-1}
\FALabel(18.4221,11.9431)[tl]{$W$}
\FAProp(20.,5.)(15.5,10.)(0.,){/Sine}{1}
\FALabel(18.4221,8.0569)[bl]{$W$}
\FAProp(4.,10.)(10.,10.)(0.,){/Sine}{0}
\FALabel(7.,11.07)[b]{$V$}
\FAProp(10.,10.)(15.5,10.)(0.8,){/ScalarDash}{0}
\FALabel(12.75,6.98)[t]{$S$}
\FAProp(10.,10.)(15.5,10.)(-0.8,){/ScalarDash}{0}
\FALabel(12.75,13.02)[b]{$S$}
\FAVert(4.,10.){0}
\FAVert(10.,10.){0}
\FAVert(15.5,10.){0}

\FADiagram{}
\FAProp(0.,15.)(4.,10.)(0.,){/Straight}{1}
\FALabel(1.26965,12.0117)[tr]{$u$}
\FAProp(0.,5.)(4.,10.)(0.,){/Straight}{-1}
\FALabel(2.73035,7.01172)[tl]{$u$}
\FAProp(20.,15.)(15.5,10.)(0.,){/Sine}{-1}
\FALabel(18.4221,11.9431)[tl]{$W$}
\FAProp(20.,5.)(15.5,10.)(0.,){/Sine}{1}
\FALabel(18.4221,8.0569)[bl]{$W$}
\FAProp(4.,10.)(10.,10.)(0.,){/Sine}{0}
\FALabel(7.,11.07)[b]{$V$}
\FAProp(10.,10.)(15.5,10.)(0.8,){/Sine}{0}
\FALabel(12.75,6.73)[t]{$V$}
\FAProp(10.,10.)(15.5,10.)(-0.8,){/Sine}{0}
\FALabel(12.75,13.27)[b]{$V$}
\FAVert(4.,10.){0}
\FAVert(10.,10.){0}
\FAVert(15.5,10.){0}

\end{feynartspicture}
\end{small}
\end{center}

